Orbifold points on Teichm\"uller curves and Jacobians with complex multiplication

For each integer $D \geq 5$ with $D \equiv 0$ or $1 \bmod 4$, the Weierstrass curve $W_D$ is an algebraic curve and a finite volume hyperbolic orbifold which admits an algebraic and isometric immersion into the moduli space of genus two Riemann surfaces. The Weierstrass curves are the main examples of Teichm\"uller curves in genus two. The primary goal of this paper is to determine the number and type of orbifold points on each component of $W_D$. Our enumeration of the orbifold points, together with work of Bainbridge and McMullen, completes the determination of the homeomorphism type of $W_D$ and gives a formula for the genus of its components. We use our formula to give bounds on the genus of $W_D$ and determine the Weierstrass curves of genus zero. We will also give several explicit descriptions of each surface labeled by an orbifold point on $W_D$.

==> appc.tex <==
\section{Surfaces with involutions}
\label{sec:properord4}
In this section we prove the facts about surfaces with involutions needed for our analysis of the $D_8$-family.
\begin{prop} 
  \label{prop:nodalproperord4}
  Fix a nodal surface $X=E \vee F$ in $\wt \M_2$ with an involution $\phi\in \Aut(X)$.  The induced action of $\zz[\phi]\cong \ord_4$ on $\jac(X)$ is proper if and only if $\phi$ interchanges the components of $X$.
\end{prop}
\begin{proof}
  First suppose $\phi$ stabilizes the components of $X$.  The induced action of $\phi$ on $\jac(X) \cong E \times F$ is by a diagonal matrix and extends to the action of $\ord_1$ by diagonal matrices $\spmat{a & 0 \\ 0 & b}$ for $(a,b) \in \zz \times \zz$.  The action of $\zz[\phi]$ is not proper.

  Conversely, suppose $\phi$ does interchange the components of $X$ and let $f$ be the isomorphism $\phi|_E : E \rightarrow F$.  The action of $\phi$ on $\jac(X) \cong E \times F$ is by the matrix $\spmat{0 & f \\ f^{-1} & 0}$ whence $\rho: \zz[\phi] \rightarrow \End(\jac(X))$ is injective.  The maximal order $\zz[(1+\phi)/2]$ is the only order properly containing $\zz[\phi]$ in $\qq[\phi]$.  Since the rational endomorphism $(1+\phi)/2$ is not integral, $\rho$ is proper.
\end{proof}

\begin{prop}
  \label{prop:smoothproperord4}
  If $X$ is a smooth genus two surface and $\phi$ is an involution on $X$ different from the hyperelliptic involution, then the induced action of $\zz[\phi] \cong \ord_4$ on $\jac(X)$ is proper.
\end{prop}
\begin{proof}
  Since $\phi$ is not the hyperelliptic involution, $\zz[\phi] \rightarrow \End(\jac(X))$ is injective.  The only order containing $\zz[\phi]$ in $\qq[\phi]$ is the maximal order $\zz[(\phi+1)/2] \cong \ord_1$, and every surface with an action of $\ord_1$ is nodal.  The action of $\zz[\phi]$ on $\jac(X)$ does not extend to a larger ring.
\end{proof}

\begin{prop}
  \label{prop:genusonequotient}
  Fix $X \in \wt \M_2$ with an involution $\phi$.  If the induced action of $\zz[\phi]$ on $\jac(X)$ is proper, then:
  \begin{enumerate}
    \item The quotient $E=X/\phi$ has genus one.
    \item The points fixed by $\eta \phi$ form a single $\phi$-orbit whose image in $E$ we take to be the base point $E[1]=\Fix(\eta \phi)/\phi$.
    \item The quotient map $X \rightarrow E$ intertwines the hyperelliptic involution $\eta$ on $X$ with the elliptic involution $\eta_E$ on $E$.
    \item The involution $\phi$ acts by a product of three disjoint transpositions on $X^W$ and the image of $X^W$ in $E$ coincides with the two torsion:
      \[ E[2]^* = X^W/\phi. \]
  \end{enumerate}
\end{prop}
\begin{proof}
  For nodal surfaces, claims $(1-4)$ follow easily from the fact that $\phi$ interchanges the components of $X$ (Proposition \ref{prop:nodalproperord4}).  The only point fixed by $\eta \phi$ is the node and $\eta$ induces an automorphism of $X/\phi$ since $\eta$ and $\phi$ commute.
  
  Now suppose $X$ is a smooth genus two surface.  Claim $(1)$ that $X/\phi$ has genus one follows from the fact that the hyperelliptic involution is the unique involution with genus zero quotient.  
  
  Since the images of the rings $\zz[\phi]$ and $\zz[\eta \phi]$ in $\End(\jac(X))$ coincide, the quotient $F=X/\eta \phi$ also has genus one.  The set $\Fix(\eta \phi)$ consists of two points which are the simple zeros of a one form obtained by pulling back a holomorphic one form on $F$.  In particular, the set $\Fix(\eta \phi)$ is disjoint from $X^W$.  Using the fact that $\phi$ and $\eta$ commute, it is easy to show that if $P \in \Fix(\eta \phi)$ then $\phi(P) \in \Fix(\eta \phi)$ and that $\phi(P) \neq P$, establishing $(2)$.  
  
  Since $\phi$ and $\eta$ commute, $\eta$ induces an involution $\eta_E$ on $E$.  The involution $\eta_E$ fixes the point $\Fix(\eta \phi)/\phi$ since the two points in $\Fix(\eta \phi)$ are the zeros of a holomorphic one form, establishing $(3)$.  Finally, to prove $(4)$, note that $\Fix(\phi)$ are the zeros of a holomorphic one form with simple zeros obtained by pulling back a one form on $E$.  In particular, $\Fix(\phi)$ is disjoint from $X^W$ and $\phi$ acts by a product of three disjoint transpositions on $X^W$.  The image of $X^W$ in $E$ consists of three points which are fixed by $\eta_E$ since $\eta$ fixes $X^W$ pointwise and $E[2]^* = X^W/\phi$.
\end{proof}

\begin{prop}
  \label{prop:jacobianproperord4}
  Fix $X \in \wt \M_2$ with an involution $\phi \in \Aut(X)$ generating a proper $\ord_4$-action on $\jac(X)$ and set $E = X / \phi$ and $F=X / \eta \phi$.  The Jacobian of $X$ satisfies:
  \[ \jac(X) \cong E \times F / \Gamma^W, \]
  where $\Gamma^W$ is the subgroup of $E[2] \times F[2]$ generated by the image of $X^W$ under $X \rightarrow E \times F$.  The principal polarization on $\jac(X)$ pulls back to twice the product polarization on $E \times F$ under the quotient by $\Gamma^W$ map.
\end{prop}
\begin{proof}
  The map $X \rightarrow E \times F$ factors through the Jacobian of $X$:
  \[ f: \jac(X) \rightarrow E \times F. \]
  The degree of $f$ is equal to the index of the image of the induced map on $H_1(X,\zz) \rightarrow H_1(E, \zz) \oplus H_1(F,\zz)$ homology.  The degree of $f$ is four, which can be computed using the fact that $H_1(X,\zz)$ is isomorphic to $\zz[\phi]\oplus\zz[\phi]$ as a $\zz[\phi]$-module (\cite{mcmullen:slrdynamics}, Theorem 4.4).  The image of $X^W$ under $X \rightarrow E \times F$ is the graph of the identifications:
  \[ E[2]^* = X^W/\phi = X^W / \eta \phi = F[2]^*. \]
  The middle equality comes from the fact that $\eta$ fixes $X^W$ pointwise.  The group $\Gamma^W$ consists of four points and coincides with the image of $\jac(X)[2]$ in $E \times F$.  Composing $f$ with the quotient by $\Gamma^W$ map gives a degree sixteen map:
  \[ \jac(X) \rightarrow E \times F / \Gamma^W, \]
  which vanishes on the two torsion and factors through the multiplication by two map on $\jac(X)$ to give an isomorphism.  
  
  The polarization on $\jac(X)$ induces a product polarization on $E \times F$ since the lines in $\Omega(X)$ pulled back from $\Omega(E)$ and $\Omega(F)$ are the eigenspaces for the self-adjoint endomorphism induced by $\phi$ and are orthogonal.  Let $\omega_E(\cdot,\cdot)$ and $\omega_F(\cdot,\cdot)$ be the unimodular polarizations on $E$ and $F$ respectively.  It is easy to check that the product of $k_1 \omega_E$ and $k_2\omega_F$ is integral on $E \times F / \Gamma^W$ if and only if both $k_1$ and $k_2$ are even and is unimmodular if and only if $k_1=k_2=2$.
\end{proof}

